TimeLens: Event-based Video Frame Interpolation

State-of-the-art frame interpolation methods generate intermediate frames by inferring object motions in the image from consecutive key-frames. In the absence of additional information, first-order approximations, i.e. optical flow, must be used, but this choice restricts the types of motions that can be modeled, leading to errors in highly dynamic scenarios. Event cameras are novel sensors that address this limitation by providing auxiliary visual information in the blind-time between frames. They asynchronously measure per-pixel brightness changes and do this with high temporal resolution and low latency. Event-based frame interpolation methods typically adopt a synthesis-based approach, where predicted frame residuals are directly applied to the key-frames. However, while these approaches can capture non-linear motions they suffer from ghosting and perform poorly in low-texture regions with few events. Thus, synthesis-based and flow-based approaches are complementary. In this work, we introduce Time Lens, a novel indicates equal contribution method that leverages the advantages of both. We extensively evaluate our method on three synthetic and two real benchmarks where we show an up to 5.21 dB improvement in terms of PSNR over state-of-the-art frame-based and event-based methods. Finally, we release a new large-scale dataset in highly dynamic scenarios, aimed at pushing the limits of existing methods.

==> chapters/notes.tex <==
\subsection{Comparisons}
\subsubsection{Comparison with SOTA Frame-based methods}
Idea is to downsample high framerate video to low framerate, run SOTA methods and evaluate on held out frames
For event-based methods we synthesize synthetic events from held-out frames (+plus frame interpolation?) then use frames + synthetic events for frame-interpolation
\subsubsection{Methods}
\begin{itemize}
    \item SepConv ICCV 2017, Code: https://github.com/sniklaus/sepconv-slomo
    \item Super SlowMo CVPR 2018 https://arxiv.org/abs/1712.00080, Code: https://github.com/avinashpaliwal/Super-SloMo, datasets: Middlebury, UCF101, sintel, slowflow
    \item DAIN CVPR 2019 - http://arxiv.org/abs/1904.00830, Code: https://github.com/baowenbo/DAIN, Datasets: EVALUATION set of the Middlebury benchmark , UCF101 [33], Vimeo90K [39], HD [2], and Middlebury OTHER dataset
    \item Flawless Video Interpolation https://github.com/MeiguangJin/slow-motion/blob/master/cvpr19.pdf, Code:https://github.com/MeiguangJin/slow-motion, Datasets: GoPro, Sony RXV
    \item TDAN CVPR 20 https://arxiv.org/pdf/1812.02898.pdf, Code: https://github.com/YapengTian/TDAN-VSR-CVPR-2020, Datasets: SPMCs-30, Vimeo SuperResolution, Vid4 benchmark
    \item Zooming SlowMo CVPR 2020 https://arxiv.org/abs/2002.11616, Code: https://github.com/Mukosame/Zooming-Slow-Mo-CVPR-2020, They do SR and interpolation. Dataset: Vimeo testset, Vid4
    \item BMBC ECCV2020 https://arxiv.org/abs/2007.12622, Code: https://github.com/JunHeum/BMBC, Datasets: Middlebury
\end{itemize}
$\rightarrow$ focus on BMBC, RRIN, DAIN, Super SlowMo\\
$\rightarrow$ datasets: Middlebury, Vimeo90k, UCF101\\
$\rightarrow$ add training dataset for each method\\

\subsubsection{Comparison with SOTA Event-based methods}
\begin{itemize}
    \item Bringing a blurry frame alive: https://openaccess.thecvf.com/content\_CVPR\_2019/papers/Pan\_Bringing\_a\_Blurry\_Frame\_Alive\_at\_High\_Frame-Rate\_With\_an\_CVPR\_2019\_paper.pdf, Code: https://github.com/panpanfei/Bringing-a-Blurry-Frame-Alive-at-High-Frame-Rate-with-an-Event-Camera, Datasets: GoPro, DAVIS event camera datasets, their own data.
    \item Deblurring and Frame interpolation, https://www.ecva.net/papers/eccv\_2020/papers\_ECCV/papers/123530681.pdf, No Code, Dasets: GoPro and Blur-DVS.
    \item Continuous Time intensity reconstruction: ACCV18, Code: https://github.com/cedric-scheerlinck/dvs\_image\_reconstruction
\end{itemize}

$\rightarrow$ add E2VID baseline
\section{TODOs}
Script for computing result  
In : (dataset, number\_of\_skips, folder, folder with in between frame events)     
Out : (folder with missing frames, e.g. 0001.png)

Script for evaluation


\subsection{Contributions}
\begin{outline}
\1 New dual dataset, high resolution, high quality.
\1 Combines advantages of traditional and fusion based:
\1 Color? High quality texture? - compare to event base
\1 Handle focus, handle light change, handle new object, nonlinearity - compare to traditional 
\end{outline}

\subsection{Ideas for a full paper}
\begin{itemize}
    \item Pretrain one frame-based method and our method on DAVIS and show results.
    \item Add score deviations to the ablation study
    \item Add graph with distribution of attention network classes.
    \item Add performance analysis for different categories: blurry videos, light change videos. 
    \item Insert visual examples that show that previous method can not handle blur and light changes and nonlinear motion. Maybe insert links to the video so when click on the image you are redirected to video.
\end{itemize}


\subsubsection{Stepan}
\begin{outline}
\1 What parts allowed to be modified after paper review by Huawei.
\1 Make patent application.
\1 Make method and intro section. 
\1 Convert Vimeo \& GoPro,
\1 Evaluate our on Vime0 GoPro..
\1 “Bring blurry frame alive” 
\1 Evaluate our HQF.
\1 Script for BMBC.
\1 Run evaluation Vimo90k
\end{outline}

\subsubsection{Daniel}
\begin{outline}
\1 Test on HQF
\1 Experimental and Related Work
\1 Evaluate frame-based mehtods (RRIN), DAIN, SuperSlowMo
\1 Evaluate E2VID, esl-method
\end{outline}

\begin{outline}
\1 Evaluation on synthetic event datasets
\2 Convert Vimeo + UCF101 + GoPro to events
\2 Compare against BMBC, DAIN, Super SlowMo
\2 Modify “Bringing a blurry frame, …”, to remove blur dependent code.
\2 Modify E2VID + Continuous to conform to frame interpolation
\1 Evaluate DAVIS dataset
\2 Run E2VID, ESL-Net, and ours on HQF.
\2 Run BMBC, DAIN, Super SlowMo on HQF
\1 Evaluate on Dual Set 
\2 Collect and calibrate.
\2 Run only our method.
\2 Most likely finetune our method
\1 Special case DAVIS / synthetic SLO MO:
\2 Refocusing, light change, non-linear motion 
\end{outline}

\subsubsection{Julius}
\begin{outline}
\0 close
\1 Training
\2 water\_bomb\_air (recrop 60, 20, 957, 857)
\2 lighting\_match
\2 fountain\_schaffhauserplatz\_01
\2 \textbf{water\_bomb\_eth\_02} (NEW)
\2 waving\_arms
\1 Testing
\2 baloon\_popping
\2 confetti
\2 spinning\_plate
\2 spinning\_umbrella
\2 water\_bomb\_floor\_01
\2 fountain\_schaffhauserplatz\_02
\2 \textbf{fountain\_bellevue2} (NEW)
\2 \textbf{water\_bomb\_eth\_01} (NEW)

\2 \textbf{candle} (NEW) very fast motion and illumination change. maybe too fast for nice ground truth. alignment and cropping in progress
\0 far\_away
\1 Training  (area w/o evetns need switch to Julius)
\2 kornhausbruecke\_letten\_rot\_z\_01
%\2 kornhausbruecke\_letten\_rot\_z\_02 (misalignement)
\2 kornhausbruecke\_rot\_x\_05
\2 kornhausbruecke\_rot\_x\_06
\2 kornhausbruecke\_rot\_y\_03
\2 kornhausbruecke\_rot\_y\_04
\2 kornhausbruecke\_rot\_z\_01
\2 kornhausbruecke\_rot\_z\_02
\2 sihl\_04
\2 tree\_03
\2 lake\_04
\2 lake\_05
\2 lake\_07
\2 lake\_08
\2 lake\_09
\2 bridge\_lake\_04
\2 bridge\_lake\_05
\2 bridge\_lake\_06 
\2 bridge\_lake\_07
\2 bridge\_lake\_08
\1 Testing
\2 kornhausbruecke\_letten\_random\_04 \2 sihl\_03 
\2 lake\_01 (visible misalignment, index 0-783 are okay)
%\2 lake\_02 (frame loss)
\2 lake\_03 
%\2 lake\_06 (visible misalignment), temporal alignment is fine
%\2 lake\_10 (visible misalignment), temp. align is fine, last frame event spike
\2 bridge\_lake\_01
%\2 bridge\_lake\_02 (frame loss)
\2 bridge\_lake\_03



\end{outline}

==> figure_tex/eyecatcher.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=1.0\columnwidth]{figures/eyecatcher.pdf}
    %\caption{Illustration of the dual camera setup. 
    %It is made up of a Prophesee Gen4 720p monochrome event camera (top) and a FLIR BlackFly S RGB camera (bottom). 
    %The cameras are both hardware synchronized and have a baseline of \SI{2.5}{\centi\meter}}
	\label{fig:eyecatcher}
\end{figure*}


==> figure_tex/rebuttal_visualization_daniel.tex <==
\begin{figure}[htbp]
	\centering
	\vspace{-2ex}
	\includegraphics[width=1\columnwidth]{figures/rebuttal/rebuttal.pdf}\vspace{-1ex}
	\caption{Complementarity of warping- and synthesis-based interpolation.}\label{fig:reb:complementarity}
\end{figure}

==> figure_tex/rebuttal_visualization_stepan.tex <==
\begin{figure*}[htbp]
	\centering

\animategraphics[width=0.25\columnwidth,autoplay,loop]{1}{figures/rebuttal/sequence_}{0}{13}%
\includegraphics[width=0.49\columnwidth]{figures/rebuttal/closeups_stepan.pdf}
\includegraphics[width=0.24\columnwidth]{figures/rebuttal/attention_stepan.pdf}
% \includegraphics[width=0.35\columnwidth]{latex/figures/rebuttal/optical_flow.pdf}

%
% 	\includegraphics[width=0.67\columnwidth]{latex/figures/fountain/fountain_closeups.pdf}%
% 	\animategraphics[width=0.41\columnwidth,autoplay,loop]{5}{latex/figures/waterbomb/waterbomb_}{1}{20}%
% 	\includegraphics[width=0.66\columnwidth]{latex/figures/waterbomb/waterbomb_closeups.pdf}\\
% 	\animategraphics[width=0.46\columnwidth,autoplay,loop]{5}{latex/figures/fountain_2/fountain_2_}{0}{21}%
% 	\includegraphics[width=0.635\columnwidth]{latex/figures/fountain_2/fountain_2_closeups.pdf}%
%     \animategraphics[width=0.385\columnwidth,autoplay,loop]{5}{latex/figures/umbrella/umbrella_}{1}{20}%
% 	\includegraphics[width=0.635\columnwidth]{latex/figures/umbrella/umbrella_closeups.pdf}\\

% \caption{Qualitative results for the proposed method and its closes competitor DAIN~\cite{bao_2019} on our Dual Event and Color Camera Dataset test sequences: ``Fountain Schaffhauserplatz''~(top-left), ``Fountain Bellevue''~(bottom-left) ``Water bomb''~(top-right) and ``Umbrella"~(bottom-right). For each sequence, the figure shows interpolation results on the left~(the animation can be viewed in Acrobat Reader) and close up interpolation results on the right. The close-ups, show input left and right frame and intermediate interpolated frames. }
	\label{fig:qualitative}
\end{figure*}
